Tevatron-for-LHC Report: Higgs

The search for Higgs bosons in both the standard model and its extensions is well under way at the Tevatron. As the integrated luminosity collected increases into the multiple inverse femptobarn range, these searches are becoming very interesting indeed. Meanwhile, the construction of the Large Hadron Collider (LHC) and its associated experiments at CERN are nearing completion. In this TeV4LHC workshop, it was realized that any experience at the Tevatron with respect to backgrounds, experimental techniques and theoretical calculations that can be verified at the Tevatron which have relevance for future measurements at the LHC were important. Studies and contributions to these efforts were made in three broad categories: theoretical calculations of Higgs production and decay mechanisms; theoretical calculations and discussions pertaining to non-standard model Higgs bosons; and experimental reviews, analyses and developments at both the Tevatron and the upcoming LHC experiments. All of these contributions represent real progress towards the elucidation of the mechanism of electroweak symmetry breaking.

==> higgs/bbhQCD/FieldOlnessSmith.tex <==
% %% LyX 1.3 created this file.  For more info, see http://www.lyx.org/.
% %% Do not edit unless you really know what you are doing.
% \documentclass[english,aps,manuscript,nofootinbib,nobibnotes]{revtex4}
% \usepackage[T1]{fontenc}
% \usepackage[latin1]{inputenc}
% \usepackage{amsmath}
% \usepackage{graphicx}
% \usepackage{amssymb}
% 
% \makeatletter
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% User specified LaTeX commands.
% \usepackage{graphicx}
% \usepackage{bm}
% \usepackage{color,colordvi}
% 
% \usepackage{babel}
% \makeatother
% \begin{document}
% 
% %\preprint{\def\msbar{$\overline{MS}$}FSU-HEP-0601??}
% %\preprint{hep-ph/yymmnnn}
% 
% 
% \title{Higgs Production in Association with Heavy Quarks: \\Issues of QCD
% Evolution and Mass Thresholds in Variable Flavor Schemes}
% \author{B. Field}
% \email{bfield@hep.fsu.edu}
% \affiliation{Department of Physics, 
%              Florida State University, 
%              Tallahassee, Florida 32306-4350, USA}
% \author{F. Olness}
% \email{olness@smu.edu}
% \affiliation{Department of Physics, 
%              Southern Methodist University, 
%              Dallas, Texas 75275-0175}
% \author{J. Smith}
% \email{smith@insti.physics.sunysb.edu}
% \affiliation{C.N. Yang Institute for Theoretical Physics, 
%              Stony Brook University,
%              Stony Brook, New York 11794-3840, USA}
% \date{February 23, 2006}
% 
% \begin{abstract}
% We examine some general issues regarding Parton Distribution Functions
% (PDFs) involving different numbers of heavy flavors. Specifically we
% compare the differences and similarities between $3$, $4$, and $5$
% flavor number scheme PDFs for lowest order (LO), next-to-leading order
% (NLO), and next-to-next-to-leading order (NNLO) evolutions.  We look
% at the implications for these different schemes and orders of
% perturbation expansions, and also study the matching conditions at the
% threshold. We use the \textsc{cteq}6 data fit as our starting point in
% comparing the different evolutions.
% \end{abstract}
% 
% \pacs{13.87.Ce, 12.38.Qk, 13.85.Ni}
% 
% \maketitle
% 
% \section{Introduction}
\emph{B. Field,$\!^{1}$ F. Olness,$\!^{2}$ J. Smith$^{3}$}\\

\noindent\emph{$^1$ Department of Physics, 
  Florida State University, 
  Tallahassee, Florida 32306-4350, USA. E-mail: bfield@hep.fsu.edu}\\
\emph{$^2$ Department of Physics, 
  Southern Methodist University, 
  Dallas, Texas 75275-0175.  E-mail: olness@smu.edu}\\
\emph{$^3$ C.N. Yang Institute for Theoretical Physics, 
  Stony Brook University,
  Stony Brook, New York 11794-3840, USA.  E-mail: smith@insti.physics.sunysb.edu}
\vspace{0.25in}

The LHC will span an unprecedented range of energies and open up new
kinematic regions for exploration and discovery. This large energy
range poses a theoretical challenge as we encounter multi-scale processes
involving many distinct energy/momentum scales. Understanding the
data that is to come from the Large Hadron Collider (LHC) in the coming
years will require a detailed and precise understanding of parton
distribution functions through next-to-next-to-leading order (NNLO). 

As we move through these different energy ranges, one can consider
implementing PDFs with varying number of flavors $N_{F}$. If our
experiments were confined to a limited energy range, a single $N_{F}$
flavor scheme would be adequate; however, since the energy scales
are widely varying, it becomes necessary to use a series of different
$N_{F}$ schemes ($N_{F}=\{3,4,5\}$) to accurately describe the entire
energy range. The question of how and where to {}``join'' these
schemes also raises significant issues
\footnote{The recent paper by Thorne\cite{Thorne:2006qt} considers
some of these issues and choices, particularly the issues that arise
at NNLO.}. While it is common to join these schemes at an energy scale
equal to the quark mass (i.e., $\mu=m_{c,b}$) since the PDFs will be
continuous (but with discontinuous derivatives) at LO and NLO with
this matching condition, we see this property is no longer true at
NNLO.


\subsubsection*{Issues of $N_{F}$ Flavor Schemes}

We can illustrate some of these issues by considering the example of
Higgs production via b-quarks in the kinematic range where the b-quark
mass is too heavy to be ignored, but too light to be decoupled from
the hadron dynamics. To work towards a solution which is valid
throughout the full energy spectrum, we start by focusing on the
asymptotic high and low energy regions (where the issues are simpler),
and then try and make these disparate regions match in the (more
difficult) intermediate region.

For example, if the characteristic energy range $\mu$ is small
compared to the b-quark mass $m_{b}$, then the b-quark decouples from
the dynamics and \textit{does not} appear as a partonic constituent of
the hadron; that is, $f_{b}(\mu<m_{b})=0$ and we are working in a
$N_{F}=4$ flavor scheme. In such a scheme, the Higgs is produced in
the ${\mathcal{O}}(\alpha_{s}^{2})$ process $gg\rightarrow H$ with
$b$-pairs in the intermediate state. Calculations in the $N_{F}=4$
flavor scheme have the advantage that they do not need to introduce
the b-quark PDF. If instead we consider energy scales much larger than
the b-quark mass ($\mu\gg m_{b}$), then we work in a $N_{F}=5$ flavor
scheme where the b-quark \textit{does} appear as a partonic
constituent of the hadron {[}$f_{b}(\mu>m_{b})>0${]}. In this regime,
the b-quark mass scale enters as powers of
$\alpha_{s}\ln(\mu^{2}/m_{b}^{2})$ which are resummed via the DGLAP
equations. This scheme has the advantage that they involve lower-order
Feynman graphs, and the $\alpha_{s}\ln(\mu^{2}/m_{b}^{2})$ terms are
resummed. Ideally, there is an intermediate region where both the
4-flavor and 5-flavor schemes are both a good representation of the
physics; in this region we can transition from the low energy 4-flavor
scheme to the high energy 5-flavor scheme thereby obtaining a
description of the physics which is valid throughout the entire energy
range from low to high scales\footnote{We label the 4-flavor and
5-flavor schemes as {}``fixed-flavor-number'' (FFN) schemes since the
number of partons flavors is fixed. The hybrid scheme which combines
these FFS is a {}``variable-flavor-number'' (VFN) scheme since it
transitions from a 4-flavor scheme at low energy to a 5-flavor scheme
at high energy\cite{Aivazis:1993pi,Aivazis:1993kh}.}.

In this report, we will focus on the different PDF's which result from
different orders of evolution (LO, NLO, NNLO) and different numbers of
active flavors ($N_{F}=\{3,4,5\}$).


\subsection{Generation of PDF Sets}

For the purposes of this study, we will start from a given set of PDFs
$f(x,Q_{0})$ at an initial scale $Q_{0}<m_{c}$. We will then evolve
the PDFs from this point and study the effect of the number of active
heavy flavors $N_{f}=\{3,4,5\}$, as well as the order of the
evolution: \{LO, NLO, NNLO\}. No fitting is involved here; the
resulting PDFs are designed to such that they are all related (within
their specific $N_{F}$-scheme and order of evolution) to be related to
the same initial PDF, $f(x,Q_{0})$. In this sense, our comparisons
will be focused on comparing schemes and evolution, rather than
finding accurate fits to data. Were we able to perform an all-orders
calculation, the choice of the number of active heavy flavors
$N_{f}=\{3,4,5\}$would be equivalent; however, since we necessarily
must truncate the perturbation expansion at a finite order, there will
be differences and some choices may converge better than others.

For our initial PDF, $f(x,Q_{0})$, we chose the \textsc{cteq}6
parametrization as given in Appendix A of
Ref.~\cite{Pumplin:2002vw}. Using the evolution program described in
Ref.~\cite{Chuvakin:2001ge}, we created several PDF tables for our
study. Essentially, we explored two-dimensions: 1) the number of
active heavy flavors $N_{f}=\{3,4,5\}$, and 2) the order of the
evolution: \{LO, NLO, NNLO\}; each of these changes effected the
resulting PDF. All the sets were defined to be equivalent at the
initial scale of $Q_{0}=m_{c}=1.3$~GeV. For the $N_{F}=3$ set, the
charm and bottom quarks are never introduced regardless of the energy
scale $\mu$. The $N_{F}=4$ set begins when the charm quark is
introduced at $\mu=m_{c}=1.3$~GeV. The $N_{F}=5$ set begins when the bottom
quark is introduced at $\mu=m_{b}=5$~GeV.

\subsubsection*{Technical Issues:}

Before we proceed to examine the calculations, let's briefly address
two technical issues.

When we evolve the b-quark PDF in the context of the DGLAP evolution
equation $df_{b}\sim P_{b/i}\otimes f_{i}$, we have the option to use
splitting kernels which are either mass-dependent
{[}$P_{b/i}(m_{b}\not=0)${]} or mass-independent
{[}$P_{b/i}(m_{b}=0)${]}. While one might assume that using
$P_{b/i}(m_{b}\not=0)$ yields more accurate results, this is not the
case. The choice of $P_{b/i}(m_{b}\not=0)$ or $P_{b/i}(m_{b}=0)$ is
simply a choice of scheme, and both schemes yield identical results up
to high-order corrections\cite{Olness:1997yn}. For simplicity, it is
common to use the mass-independent scheme since the $P_{b/i}(m_{b}=0)$
coincide with the $\overline{\textrm{MS}}$ kernels.

When the factorization proof of the ACOT scheme was extended to
include massive quarks, it was realized that fermion lines with an
initial or internal {}``cut'' could be taken as
massless\cite{Kramer:2000hn}. This simplification, referred to as the
simplified-ACOT (S-ACOT) scheme, is \textit{not} an approximation; it
is again only a choice of scheme, and both the results of the ACOT and
S-ACOT schemes are identical up to high-order
corrections\cite{Collins:1998rz}. The S-ACOT scheme can lead to
significant technical simplifications by allowing us to ignore the
heavy quark masses in many of the individual Feynman diagrams.  We
show how we exploit this feature in the case of NNLO calculation of
$b\bar{b}\rightarrow H$ in the next section.


\subsubsection*{Consistency Checks}

We first recreated the published \textsc{cteq}6 table to check our
evolution program and found excellent agreement. The evolution program
was also checked against the output described and cataloged in
Ref.~\cite{giele:2002hx} and was found to be in excellent agreement
(generally five decimal places) for all three orders when run with the
same inputs\footnote{The NNLO results presented here and in
Ref.~\cite{giele:2002hx} used an approximate form for the three-loop
splitting functions since the exact results were not available when
the original programs were produced\cite{Chuvakin:2001ge}. A
comparison of the NNLO splitting functions finds the approximate quark
distributions underestimate the exact results by at most a few percent
at small x ($x<10^{-3}$), and overestimate the gluon distributions by
about half a percent for $\mu=100$~GeV\cite{Dittmar:2005ed}. This
accuracy is sufficient for our preliminary study; the evolution
program is being updated to include the exact NNLO kernels.}.


\subsubsection*{Matching Conditions}

A common choice for the matching between $N_{F}$ and $N_{F+1}$ schemes
is to perform the transition at $\mu=m$. To be specific, let us
consider the transition between $N_{F}=3$ and $N_{F}=4$ flavors at
$\mu=m_{c}$.  If we focus on the charm ($f_{c}$) and gluon ($f_{g}$)
PDFs, the boundary conditions at NNLO can be written schematically
as\footnote{Here we use the short-hand notation $f^{N_{F}}$ for the
$N_{F}$ flavor PDF.}:
\[
f_{c}^{4}\sim f_{g}^{3}\otimes\left\{
0+\left(\frac{\alpha_{s}}{2\pi}\right)\, P_{g\rightarrow
q}^{(1)}\left(L+a_{g\rightarrow
q}^{1}\right)+\left(\frac{\alpha_{s}}{2\pi}\right)^{2}\,
P_{g\rightarrow q}^{(2)}\left(L^{2}+L+a_{g\rightarrow
q}^{2}\right)+O(\alpha_{s}^{3})\right\} 
\]

\[
f_{g}^{4}\sim f_{g}^{3}\otimes\left\{
1+\left(\frac{\alpha_{s}}{2\pi}\right)\, P_{g\rightarrow
g}^{(1)}\left(L+a_{g\rightarrow
g}^{1}\right)+\left(\frac{\alpha_{s}}{2\pi}\right)^{2}\,
P_{g\rightarrow g}^{(2)}\left(L^{2}+L+a_{g\rightarrow
g}^{2}\right)+O(\alpha_{s}^{3})\right\}
\]
where $L=\ln(\mu^{2}/m_{q}^{2})$ and $m_{q}=m_{c}$. Because the terms
$L=\ln(\mu^{2}/m_{q}^{2})$ vanish when $\mu=m$, the above conditions
are particularly simple at this point.

An explicit calculation shows that $a_{g\rightarrow q}^{1}=0$ and
$a_{g\rightarrow g}^{1}=0$. Consequently, if we perform the matching
at $\mu=m$ where $L=0$, we have the continuity condition
$f_{c}^{4}(x,\mu=m_{c})=f_{c}^{3}(x,\mu=m_{c})=0$ and
$f_{g}^{4}(x,\mu=m_{c})=f_{g}^{3}(x,\mu=m_{c})$. Therefore, the PDFs
will be continuous at LO and NLO.

This is no longer the case at NNLO. Specifically, the ${\cal
O}(\alpha_{s}^{2})$ coefficients $a_{g\rightarrow q}^{2}$ and
$a_{g\rightarrow g}^{2}$ have been calculated in
Ref.~\cite{Buza:1995ie} and found to be non-zero. Therefore we
necessarily will have a discontinuity no matter where we choose the
matching between $N_{3}$ and $N_{4}$ schemes; $\mu=m_{c}$ is no longer
a {}``special'' transition point. This NNLO discontinuity changes the
boundary value of the differential equations that govern the evolution
of the partons densities, thus changing the distributions at all
energy levels; these effects then propagate up to higher scales.

It is interesting to note that there are similar discontinuities in
the fragmentation function appearing at NLO. For example the NLO heavy
quark fragmentation function first calculated by Nason and
Mele\cite{Mele:1990yq}
\[
d_{c\to c}\sim\left\{
\delta(1-x)+\left(\frac{\alpha_{s}}{2\pi}\right)\, P_{c\rightarrow
c}^{(1)}\left(L+a_{c\to c}^{1}\right)+O(\alpha_{s}^{2})\right\} 
\]
found the $a_{c\to c}^{1}$ coefficient was non-zero. Additionally, we
note that $\alpha_{S}(\mu,N_{F})$ is discontinuous across flavor
thresholds at order $\alpha_{S}^{3}$\cite{Eidelman:2004wy}:
\[
\alpha_{S}(m;N_{f})=\alpha_{S}(m;N_{f}-1)-\frac{11}{72\pi^{2}}\,
\alpha_{S}^{3}(m;N_{f}-1)+O\left(\alpha_{S}^{4}(m;N_{f}-1)\right)
\]
Note that the NNLO matching conditions on the running coupling
$\alpha_{s}(N_{F},Q^{2})$ as $Q^{2}$ increases across heavy-flavor
flavor thresholds have been calculated in \cite{Bernreuther:1981sg,
Bernreuther:1983zp} and \cite{Larin:1994va, Chetyrkin:1997sg}.


\subsection{Comparison of 3,4, and 5 Flavor Schemes}


\subsubsection*{Momentum fraction and luminosity}

%
\begin{figure}
\begin{center}\includegraphics[%
  width=0.45\linewidth]{higgs/bbhQCD/new2.eps}\includegraphics[%
  width=0.45\linewidth]{higgs/bbhQCD/new1.eps}\end{center}


\caption{a) Integrated momentum fraction, $\int_{0}^{1}xf_{g}(x,\mu)\,
dx$ vs. $\mu$ of the gluon for $N_{F}=\{3,4,5\}$ = \{Red, Green,
Blue\}. b) The ratio of the gluon-gluon luminosity
($d{\mathcal{L}}_{gg}/d\tau$) vs. $\tau$ for $N_{F}=\{3,4,5\}$ =
\{Red, Green, Blue\} as compared with $N_{F}=4$ at $\mu=120$~GeV.}

\label{fig:fredi}
\end{figure}
%
\begin{figure}
\begin{center}\includegraphics[%
  width=0.45\linewidth]{higgs/bbhQCD/fredFig5.eps}\includegraphics[%
  width=0.45\linewidth]{higgs/bbhQCD/fredFig6.eps}\end{center}


\caption{$\alpha_{s}$ vs. $\mu$ (in GeV) for $N_{F}=\{3,4,5\}$ (for
large $Q$, reading bottom to top: red, green, blue, respectively)
flavors. Fig. a) illustrates the region where $\mu$ is comparable to
the quark masses to highlight the continuity of $\alpha_{S}$ across the
mass thresholds at $m_c=1.3$~GeV and  $m_b=5$~GeV. 
Fig. b) extrapolates this to larger $\mu$ scale. }

\label{fig:alphas}
\end{figure}
 To illustrate how the active number of {}``heavy'' flavors affects
the {}``light'' partons, in Fig.~\ref{fig:fredi}a) we show the
momentum fraction of the gluon vs. $\mu$. We have started with a
single PDF set at $\mu=1.3$~GeV, and evolved from this scale invoking
the {}``heavy'' flavor thresholds as appropriate for the specified
number of flavors. While all three PDF sets start with the same
initial momentum fraction, once we go above the charm threshold
($m_{c}=1.3$~GeV) the $N_{F}=\{4,5\}$ gluon momentum fractions are
depleted by the onset of a charm quark density. In a similar fashion,
the gluon momentum fraction for $N_{F}=5$ is depleted compared to
$N_{F}=4$ by the onset of a bottom quark density above the bottom
threshold ($m_{b}=5$~GeV).

To gauge the effect of the different number of flavors on the cross
section, we compute the gluon-gluon luminosity which is defined as
$d{\mathcal{L}}_{gg}/d\tau=f_{g}\otimes f_{g}$. We choose a scale of
$\mu=120$~GeV which is characteristic of a light Higgs. In terms of
the luminosity, the cross section is given as
$d\sigma/d\tau\sim[d{\mathcal{L}}_{gg}/d\tau]\,[\hat{\sigma}(\hat{s}=\tau
s)]$ with $\tau=\hat{s}/s=x_{1}x_{2}$.

To highlight the effect of the different $N_{F}$ PDF's, we plot the
ratio of the luminosity as compared to the $N_{F}=4$ case,
\textit{c.f.}, Fig.~\ref{fig:fredi}b). We see that the effects of
Fig.~\ref{fig:fredi}a) are effectively squared (as
expected---$f_{g}\otimes f_{g}$) when examining the thin lines of
Fig.~\ref{fig:fredi}b).

However, this is not the entire story. Since we are interested in
$gg\rightarrow H$ which is an $\alpha_{s}^{2}$ process, we must also
take this factor into account. Therefore we display
$\alpha_{s}^{2}(\mu,N_{F})$ computed at NLO for $N_{f}=\{3,4,5\}$ as a
function of $\mu$ in Fig.~\ref{fig:alphas}. Note at this order,
$\alpha_{s}^{2}(\mu,N_{F})$ is continuous across flavor
boundaries. Fig.~\ref{fig:alphas} explicitly shows that
$\alpha_{s}(m_{c},3)=\alpha_{s}(m_{c},4)$ and
$\alpha_{s}(m_{b},4)=\alpha_{s}(m_{b},5)$.  Comparing
Figs.~\ref{fig:fredi} and~\ref{fig:alphas} we observe that the
combination of the $N_{F}$ and $\alpha_{s}$ effects tend to compensate
each other thereby reducing the difference. While these simple
qualitative calculations give us a general idea how the actual cross
sections might vary, a full analysis of these effects is required to
properly balance all the competing factors. However, there are
additional considerations when choosing the active number of flavors,
as we will highlight in the next section.


\subsubsection*{Resummation}

%
\begin{figure}
\begin{center}\includegraphics[%
  width=0.45\linewidth]{higgs/bbhQCD/fredFig3.eps}\includegraphics[%
  width=0.45\linewidth]{higgs/bbhQCD/fredFig4.eps}\end{center}


\caption{Comparison of the evolved PDFs, $f_{b}(x,\mu)$ (labeled PDF),
and perturbative PDFs, $\widetilde{f}_{b}(x,\mu)\sim P_{b/g}\otimes
f_{g}$ (labeled SUB), as a function of the renormalization scale $\mu$
for bottom at a) $x=0.1$ and b) $x=0.01$. Taken from
Ref.~\cite{Olness:1997yc} }

\label{fig:fredii}
\end{figure}
 

%
\begin{figure}
\begin{center}\includegraphics[%
  width=0.45\linewidth]{higgs/bbhQCD/fig3cx1.eps}\includegraphics[%
  width=0.45\linewidth]{higgs/bbhQCD/fig3cx01.eps}\end{center}


\caption{Comparison of the evolved PDFs, $f_{c}(x,\mu)$ (labeled PDF),
and perturbative PDFs, $\widetilde{f}_{c}(x,\mu)\sim P_{c/g}\otimes
f_{g}$ (labeled SUB), as a function of the renormalization scale $\mu$
for charm at a) $x=0.1$ and b) $x=0.01$. Taken from
Ref.~\cite{Olness:1997yc} }

\label{fig:fredcharm}
\end{figure}


The fundamental difference between the $gg\rightarrow H$ process and
the $b\bar{b}\rightarrow H$ amounts to whether the radiative
splittings (e.g., $g\rightarrow b\bar{b}$) are computed by the DGLAP
equation as a part of the parton evolution, or whether they are
external to the hadron and computed explicitly. In essence, both
calculations are represented by the same perturbation theory with two
different expansion points; while the full perturbation series will
yield identical answers for both expansion points, there will be
difference in the truncated series.

To understand source of this difference, we examine the contributions
which are resummed into the b-quark PDF by the DGLAP evolution
equation, $df\sim P\otimes f$. Solving this equation perturbatively in
the region of the b-quark threshold, we obtain $\widetilde{f}_{b}\sim
P_{b/g}\otimes f_{g}$.  This term simply represents the first-order
$g\rightarrow b\bar{b}$ splitting which is fully contained in the
${\mathcal{O}}(\alpha_{s}^{2})$ $gg\rightarrow H$ calculation.

In addition to this initial splitting, the DGLAP equation resums an
infinite series of such splittings into the non-perturbative evolved
PDF, $f_{b}$. Both $f_{b}$ and $\widetilde{f}_{b}$ are shown in
Fig.~\ref{fig:fredii} for two choices of $x$.\cite{Olness:1997yc} Near
threshold, we expect $f_{b}$ to be dominated by the single splitting
contribution, and this is verified in the figure. In this region,
$f_{b}$ and $\widetilde{f}_{b}$ are comparable, and we expect the
4-flavor $gg\rightarrow H$ calculation should be reliable in this
region. As we move to larger scales, we see $f_{b}$ and
$\widetilde{f}_{b}$ begin to diverge at a few times $m_{b}$ since
$f_{b}$ includes higher-order splitting such as $\{
P^{2},P^{3},P^{4},...\}$ which are not contained in
$\widetilde{f}_{b}$. In this region, we expect the 5-flavor
$b\bar{b}\rightarrow H$ calculation should be most reliable in this
region since it resums the iterative splittings. For comparison,
$f_{c}$ and $\widetilde{f}_{c}$ are shown in Fig.~\ref{fig:fredcharm}
which have similar behavior.


\subsubsection*{NNLO\label{sec:NNLO}}

The fixed-flavor NLO QCD corrections to charm quark electro-production
were calculated in Ref.~\cite{Laenen:1992zk} in the three-flavor
scheme. The treatment of the heavy quark as a parton density requires
the identification of the large logarithmic terms $\log(Q^{2}/m^{2})$,
which was done in Ref.~\cite{Buza:1995ie} through next-to-next-leading
order (NNLO). Then based on a two-loop analysis of the heavy quark
structure functions from an operator point of view, it was shown in
Refs.~\cite{Buza:1997nv}, \cite{Buza:1996wv} and
\cite{Matiounine:1998ky} how to incorporate these large logarithms
into charm (and bottom) densities. Two different NNLO variable flavor
number schemes were defined in Refs.~\cite{Chuvakin:2000jm} and
\cite{Chuvakin:1999nx}, where it was shown how they could be matched
to the three-flavor scheme at small $Q^{2}$, the four-flavor scheme at
large $Q^{2}$, and the five-flavor scheme at even larger $Q^{2}$.

This NNLO analysis yielded two important results. One was the complete
set of NNLO matching conditions for massless parton evolution between
$N$ and $N+1$ flavor schemes. Unlike the LO and NLO case, the NNLO
matching conditions are discontinuous at these flavor thresholds.
Such matching conditions are necessary for any NNLO calculation at the
LHC, and have already been implemented in parton evolution packages by
\cite{Chuvakin:2001ge}, \cite{Vogt:2004ns}.

%
\begin{figure}
\begin{center}\includegraphics[%
  scale=0.3,
  angle=-90]{higgs/bbhQCD/bottom2.ps}\includegraphics[%
  scale=0.3,
  angle=-90]{higgs/bbhQCD/bot_compare.ps}\end{center}


\caption{a) Comparison of the NNLO evolved PDFs, $f_{b}(x,\mu)$
vs. $Q^{2}$ using the NNLO matching conditions at$\mu=m_{b}$ for three
choices of x values: $\{10^{-3},10^{-4},10^{-5}\}$. b) Comparing
$f_{b}(x,\mu)$ vs. $Q^{2}$ for three orders of evolution \{LO, NLO,
NNLO\} at $x=0.01$. In this figure we have set $m_{b}=4.5$~GeV.
\label{fig:bottom}}
\end{figure}


%
\begin{figure}
\begin{center}\includegraphics[%
  scale=0.3,
  angle=-90]{higgs/bbhQCD/gluon2.ps}\includegraphics[%
  scale=0.3,
  angle=-90]{higgs/bbhQCD/glu_compare.ps}\end{center}


\caption{a) Comparison of the NNLO evolved PDFs, $f_{g}(x,\mu)$
vs. $Q^{2}$ using the NNLO matching conditions at$\mu=m_{b}$ for three
choices of x values: $\{10^{-3},10^{-4},10^{-5}\}$. b) Comparing
$f_{g}(x,\mu)$ vs. $Q^{2}$ for three orders of evolution \{LO, NLO,
NNLO\} at $x=0.01$. In this figure we have set $m_{b}=4.5$~GeV.
\label{fig:gluon}}
\end{figure}


We illustrate this property in Figs.~\ref{fig:bottom} and
\ref{fig:gluon}.  In Fig.~\ref{fig:bottom}, we see that $f_{b}(x,\mu)$
vanishes for $\mu<m_{b}$; however, due to the non-vanishing NNLO
coefficients, we find $f_{b}(x,\mu)$ is non-zero (and negative) just
above the $m_{b}$ scale. This leads to a ${\cal O}(\alpha_{S}^{2})$
discontinuity in the b-quark PDF when making the transition from the
$N_{F}=4$ to $N_{F}=5$ scheme. Additionally, note that the value of
the discontinuity is $x$-dependent; hence, there is no simple adjustment
that can be made here to restore continuity. We also observe that
there is a discontinuity in the gluon PDF across the $N_{F}=4$ to
$N_{F}=5$ transition. While the PDF's have explicit discontinuities at
${\cal O}(\alpha_{S}^{2})$, the net effect of these NNLO PDF
discontinuities will compensate in any (properly calculated) NNLO
physical observable such that the final result can only have
discontinuities of order ${\cal O}(\alpha_{S}^{3})$.

Finally, we note that the NNLO two-loop calculations above explicitly
showed that the heavy quark structure functions in variable flavor
approaches are not infrared safe. A precise definition of the
heavy-flavor content of the deep inelastic structure function requires
one to either define a heavy quark-jet structure function, or
introduce a fragmentation function to absorb the uncanceled infrared
divergence. In either case, a set of contributions to the inclusive
light parton structure functions must be included at NNLO.


\subsection{Conclusions}

While an exact {}``all-orders'' calculation would be independent of
the number of active flavors, finite order calculations necessarily
will have differences which reflect the higher-order uncalculated
terms. To study these effects, we have generated PDFs for
$N_{F}=\{3,4,5\}$ flavors using \{LO, NLO, NNLO\} evolution to
quantify the magnitude of these different choices. This work
represents an initial step in studying these differences, and
understanding the limitations of each scheme.


\subsection*{Acknowledgements}

We thank John Collins and Scott Willenbrock for valuable discussions.
F.I.O acknowledge the hospitality of Fermilab and BNL, where a portion
of this work was performed. This work is supported by the
U.S. Department of Energy under grants DE-FG02-97ER41022 and
DE-FG03-95ER40908, the Lightner-Sams Foundation, and by the National
Science Foundation under grant PHY-0354776.

%\bibliographystyle{plain}
%\bibliography{FieldOlnessSmith}

%\end{document}



==> titlepage.tex <==
\begin{titlepage}


\hbox to\hsize{\null}


\vfill
\begin{center}

\begin{LARGE}
{\bf
Final Report of \\[1ex]
TeV4LHC Workshop}
\end{LARGE}

\vfill



\vfill\vfill

\begin{Large}
January 2006\\[2ex]
Fermilab\\


\vfill\vfill \vfill


Editors\\
  M. Carena and S. Mrenna\\
\end{Large}
\vfill\vfill

 Organized by the Fermi National Accelerator Laboratory \\[2ex]

Sponsored by ????

\end{center}


\end{titlepage}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

